Automatic Generation of Formula Simplifiers based on Conditional Rewrite Rules

This paper addresses the problem of creating simplifiers for logic formulas based on conditional term rewriting. In particular, the paper focuses on a program synthesis application where formula simplifications have been shown to have a significant impact. We show that by combining machine learning techniques with constraint-based synthesis, it is possible to synthesize a formula simplifier fully automatically from a corpus of representative problems, making it possible to create formula simplifiers tailored to specific problem domains. We demonstrate the benefits of our approach for synthesis benchmarks from the SyGuS competition and automated grading.

==> alg_opt.tex <==
\begin{algorithm}[H]
     \scriptsize
     \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
     \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
     \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
     \Input{\TRAIN,\evalTRAIN,\evalRewritten}
     \Output{optimization value}
     %$ \evalTRAIN \gets \evaluate(\TRAIN)$ \\
     %$\rewriter \gets \genRewriter(rules)$\\
     %$\rewrittenTRAIN \gets \rewriter(\TRAIN)$ \\ 
     %$\evalRewritten \gets \evaluate(\simplify(\TRAIN))$ \\
	 %$\perfSum \gets  0.0$ \\
     \For{$i \gets 0  { ; } i < \sizefn(\TRAIN) { ; } i{+}{+}$}{
     	$\improved \gets \frac{\evalRewritten{[i]}}{\evalTRAIN{[i]}}$ \\
        %$\perf \gets 0.0$ \\
        \Switch{$\improved$}{
        	\Case{ < 0.5 }{
            	$\perf \gets \frac{-5.0}{\improved}$
            }
            \Case{ < 1.0 }{
            	$\perf \gets -5.0$
            }
            \Case{ < 2.0 }{
            	$\perf \gets +2.0$
            }
            \Case{ < 3.0 }{
            	$\perf \gets +3.0$
            }
            \Other{
            	$\perf \gets \improved$
            }
        }
        $\perfSum \gets \perfSum + \perf$
     }
     Output $\frac{\perfSum}{\sizefn(\TRAIN)}$
     \caption{\footnotesize Evaluation function ($\performanceFunction$) }
     \label{alg:perffn}
    \end{algorithm}

==> overview_pic.tex <==
\centering
\begin{tikzpicture}[node distance = 2cm, auto]
    % Place nodes
    \node [block, text width=5.75em] (pattern) {\scriptsize Pattern Finding \tiny (Sampling, Clustering)};
    \node [block, right of=pattern, text width=5.75em, node distance=3.5cm] (rulegen) {\scriptsize Rule Generation \tiny (Sketch Synthesis)};
    \node [block, right of=rulegen,text width=5.5em, node distance=3cm] (simplifier) { \scriptsize Simplifier Generation \tiny (Compilation)};
    \node [block, right of=simplifier, text width=5.5em, node distance = 3.5cm] (tuner) { \scriptsize Auto-tuning \tiny (Machine Learning)};
          
    \node [text centered, above of=pattern, text width=4em, node distance=1.5cm] (bench1) {\tiny Corpus of Benchmarks} ;     
    \node [text centered, below of=tuner, text width=4em, node distance=1.5cm] (optimal) {\tiny Optimal Simplifier} ;  
     
    % Draw edges
    \path [line] (bench1) edge (pattern);
 
    \path [line] (pattern) edge node [label, text width=3em] {\tiny Patterns %with static analyses' info
    } (rulegen);
    \path [line] (rulegen) edge node [label] {\tiny Rules} (simplifier);
    \path [line] (simplifier)  edge [out=10,in=170] node [label,above=0.1cm] {\tiny Simplifier} (tuner);
    \path [line] (tuner) edge [out=-170,in=-10]  node [label,below=1cm] {\tiny Subset of Rules} (simplifier);
    \path [line] (tuner) edge (optimal);
    
\end{tikzpicture}
\caption{Overall steps for \tool{}.}
    \figlabel{solution_steps}


